BAKUP: Automated, Flexible, and Capital-Efficient Insurance Protocol for Decentralized Finance

This paper introduces BAKUP, a smart contract insurance design for decentralized finance users to mitigate risks arising from platform vulnerabilities. While providing automated claim payout, BAKUP utilizes a modular structure to harmonize three key features: the platform's resilience against vulnerabilities, the flexibility of underwritten policies, and capital efficiency. An immutable core module performs capital accounting while ensuring robustness against external vulnerabilities, a customizable oracle module enables the underwriting of novel policies, and an optional and peripheral yield module allows users to independently manage additional yield. The implementation incorporates binary conditional tokens that are tradable on automated market maker (AMM)-based exchanges. Finally, the paper examines specific liquidity provision strategies for the conditional tokens, demonstrating that a conservative strategy and parameterization can effectively reduce the divergence loss of liquidity providers by more than 47 % compared to a naive strategy in the worst-case scenario.

==> design-multi-token.tex <==
\section{Protocol Design}\label{sec:design}
\textbf{This version is for journal.}
The protocol design is modular, with key components divided into the \emph{core} and \emph{periphery} modules. The design of the core module is such that it enables interaction with the periphery modules. The periphery modules can either be existing smart contract applications or custom-built.
Here is a detailed explanation of each of these modules:
\subsection{Event}
We define \emph{singular event} $\E(\A, s, T)$ with the following set of parameters:
\begin{itemize}
    \item Assertion: An event is characterized by an immutable assertive statement $\A$. For example, $p_{stETH/ETH}<0.95$.
    \item Expiration period $T$: This represents the time duration since the inception of an event during which it remains valid. After the expiration period has passed, the current state of the event becomes immutable, as explained next.
    \item State: An event has two states: \emph{True} and \emph{False}. By default, an event is in the \emph{False} state. If the underlying assertion statement becomes valid at any time before the event's expiration, the state shifts to \emph{True} and becomes immutable.
\end{itemize}
Since there are only two possible states for an event, each of the singular events shall also be referred to as \emph{Binary} events.

We model an adversity as a composition of $n\in \mathbb{N}$ singular events $\E_{1}, \E_{2},\ldots \E_{n}$ with the same expiry period $T$ and denote it by $\E_{1}\times \E_{2} \ldots \times \E_{n}$. 

\subsection{Core Module}
For an adversity $\E_{1}\times \E_{2} \ldots \times \E_{N}$, the core module creates $N+1$ ERC20 tokens denoted by $\K_{i}$ with $i \in [1,N]$, and $\I$. Each core contract is characterized by a base currency $\C$ (for \emph{eg.,} ETH, USDC \emph{etc.}) in which claims are disbursed. From the inception of the core module to perpetuity, the following invariant holds:
\begin{equation}\label{inv}
    \sum_{i=1}^{N}\K_{i} + \I = N\cdot \C
\end{equation}
This is implemented as follows: 
\begin{enumerate}
    \item \texttt{Mint:} A user depositing $n$ units of $\C$ receives $n/N$ units of $\K_{i}$ $ \forall i\in [1,N]$ and $n/N$ units of $\I$.
    \item \texttt{Burn:} A user depositing $n/N$ units of $\K_{i}$ $\forall i\in [1,N]$ and $n/N$ units of $\I$ receives $n$ units of $\C$.
    
\end{enumerate}
Let $\R\subseteq [1,N]$ denote the set of events whose state is set to \emph{True}. Then at any point in time, $\K_{i}$ $ \forall i\in \R$ can be redeemed for $1-\epsilon$ units of $\C$ tokens using \texttt{Redeem()} method. Here, $0 < \epsilon < 1 $ is a constant, and generally close to zero. After the core contract expires, the \texttt{Redeem()} function can be used to redeem either $\K$ or $\I$ in exchange for the following:
\begin{itemize}
    \item $1-\epsilon$ units of $\C$ for $\K_{i}$ $ \forall i\in \R$. 
    \item $\epsilon$ units of $\C$ for $\K_{i}$ $ \forall i\in [1,N]\setminus \R$.
    \item $N-|\R|+\epsilon\cdot (2|\R|-N)$ units of $\C$ for $\I$.
\end{itemize}
The above redeem values satisfy the Invariant~\ref{inv}. This has the following interpretation: if an adverse event $\E_{j}$ occurs before the contract's deadline, the holder of $1$ $\K_{j}$ is entitled for $1-\epsilon$ units of $\C$. Otherwise, they are entitled for $\epsilon$ units of $\C$. This creates a hedging mechanism for the holder of $\K_{j}$ against adversity $\E_{j}$. On the other hand, after the contract expires, the holder of $\I$ is entitled for $N-R +\epsilon\cdot (2R-N)$ units of $\C$, where $R$ out $N$ adverse events occur. Therefore, the holder of $\I$ is providing hedging against adverse events to the holders of $\K$.

\if 0
Moreover, it enforces the following relation:
\begin{equation}
    \I \ge R\cdot \C
\end{equation}
\fi 

The core module also consists of a \texttt{Trigger(j)} function with the argument $j$ belonging to the domain $[1,N]$. This function executes the callback function in the Oracle contract. The Oracle contract executes the logic of the assertive statement $\A$ for the binary event $\E_{j}$. If the assertion holds true, the callback returns \emph{True} leading to the following consequences:
\begin{enumerate}
    \item The state of $\E_{j}$ transitions to \emph{True}.
    \item $\E_{j}$ is included in the set $\R$ and $|\R|$ increases by $1$.
    \item The \texttt{RedeemT(j)} method is set to exchange $\epsilon\cdot \C$ for $1\K_{j}$ when called.
\end{enumerate}

When the contract deadline passes, the following set of actions occur:
\begin{enumerate}
    \item The \texttt{Trigger()} method is rendered invalid.
    \item $\R$ becomes immutable.
    \item The \texttt{RedeemT(j)} function becomes valid $\forall j \in [1,N]$ redeeming $\C$ as defined before.
\end{enumerate}
\subsection{Oracle Module}
The Oracle contract is an externally deployed contract that consists of developer-defined logic to implement the assertion statement for each event.

When someone creates the core contract on {\name}, they specify the Oracle contract during deployment. The \texttt{Trigger(j)} method in the core contract calls the \texttt{OTrigger(j)} method of the Oracle contract. After completing this method, the callback is executed in the Core contract. This is presented as a flowchart diagram in Figure~\ref{fig:backup-oracle-flow}.
Such a design gives the flexibility to encode all types of assertion statements, in both permissioned and permissionless way. External information such as prices, liquidity, \emph{etc.}, can be sampled from either on-chain or off-chain oracle sources. Therefore, the design of the oracle contract can range from being
\begin{itemize}
    \item \textbf{Centralized} by utilizing oracle solutions such as Chainlink, or \textbf{decentralized} using solutions such as Time Weighted Average Price (TWAP) in AMMs such as Uniswap V3, or a mix of both.
    \item \textbf{Permissionless} by allowing anyone to update the oracle values, or \textbf{permissioned} by allowing certain trusted addresses to call the update function.
\end{itemize}
\begin{figure}[h]
\includegraphics[width=9cm]{img/Backup-oracle-flowchart.pdf}
\caption{Flow of Trigger execution using Oracle module.}
\label{fig:backup-oracle-flow}
\end{figure}
\textbf{Should also talk about fee sharing with oracle deployer}
{\name} protocol
\begin{figure}[h]
\includegraphics[width=10cm]{img/Backup-modules.pdf}
\caption{Core and periphery modules of the {\name} protocol.}
\label{fig:backup-module}
\end{figure}
\subsection{Token Marketplace}
Suppose there are $N$ adversarial events $\E_{1},\E_{2},\ldots \E_{N}$ for which we want to create insurance tokens. There are two ways to achieve this: \emph{(a)} By creating $N$ core contracts thus creating $N$ pairs of $\K_{i},\I_{i}$ tokens, or \emph{(b)} By creating one core contract with $N$ $\K_{i}$ and one $\I$ token.

The second method is more capital efficient using DEEPER.
Next, we need to define the LP strategy for both of the cases. And then evaluate it in the next section.


There are two kinds of token involved in the working of the {\name} protocol:
\begin{enumerate}
    \item Token $I$, which is held by risk-taking users willing to provide insurance against an adverse event $\E_{i}$ in exchange for a premium.
    \item Token $\K_{i}$, which is held by the risk-averse users who are willing to pay a fee to hedge against the adverse event $\E_{i}$.  
\end{enumerate}
For a proper functioning of the {\name} protocol, it is important to have an efficient marketplace where a user can buy or sell $\I$ and $\K_{i},$ $i\in [1,N]$ in exchange for a common currency such as $\C$. An important consideration for such a marketplace is capital-efficient liquidity provision \emph{i.e.,} providing higher liquidity using same amount of asset reserves. Therefore, we propose using a shared concentrated liquidity DEX such as \textbf{DEEPER (put it as an add-on otherwise, reviewers might not understand the paper)} on the $N$ trading pairs $\K_{i}/\I$ with $\I$ being the common token. Compared to having $N$ separate pools, one for each trading pair $\K_{i}/\I$, the shared liquidity model enhances the liquidity of $\I$.

For a given $\textbf{j}$, a user willing to buy $1$ $\K_{\textbf{j}}$ can performing the following ordered actions in a single transaction:
\begin{enumerate}
    \item Take a flash loan of $N\cdot \C$.
    \item Mint $\K_{i}$ $\forall i \in [1,N]$ and $\I$ using $N\cdot \C$.
    \item Sell $\K_{i}$ $\forall i \in [1,N]\setminus \{\textbf{j}\}$ and $\I$ for $N'\cdot \C$.
    \item Pay $\mathit{max}(N-N',0)$ and return the flash loan.
\end{enumerate}
Similar can be done when the user wants to sell $\K_{\textbf{j}}$ by taking a flash loan of $N'\cdot \C$, buying $\K_{i}$ $\forall i \in [1,N]\setminus \{\textbf{j}\}$ and $\I$ for $N'\cdot \C$, burning the gathered tokens for $N\cdot \C$, and then returning $N'\cdot \C$. At the end, the user gets to keep $\mathit{max}(N-N',0)$.

At any point in time, let $\rho_{i}\in [0,1]$ denote the probability of $\E_{i}$ occurring, then the fair price $p^{*}_{i,\C}$ of $\K_{i}/\C$ and $p^{*}_{\I,\C}$ of $\I/\C$ is:
\begin{equation}
\begin{split}
        p^{*}_{i,\C} = (\rho_{i}(1-\epsilon) +(1-\rho_{i}) \epsilon)\cdot\C\\
        p^{*}_{\I,\C} = N\cdot \C -\sum_{i=1}^{N} p^{*}_{i,\C}
\end{split}
\end{equation}
Here, we used that $\sum_{i=1}^{N} p^{*}_{i,\C}+p^{*}_{\I,\C}=N\cdot\C$ using Invariant~\ref{inv}. Ignoring the risk-free interest rate on $\C$, the actual price $p_{i,\C}$ for each pair $\K_{i}/\C$, and $p_{\I,\C}$ for $\I/\C$ should satisfy:
\begin{equation}
\begin{split}
      \epsilon\cdot\C\le p_{i,\C}\le (1-\epsilon)\cdot \C\\
      N\epsilon\cdot\C\le p_{\I,\C} \le N(1-\epsilon)\cdot\C
\end{split}
\end{equation}
This is because if $p_{i,\C}< \epsilon\cdot\C$ or $p_{\I,\C}< N\epsilon\cdot\C$, then a trader can buy these tokens at a cheaper price and sell them at a higher price when the contract expires, thus creating an arbitrage over time. Similarly, if $p_{\I,\C}>N(1-\epsilon)\cdot\C$, Invariant~\ref{inv} implies that $\exists j$ $s.t.$ $p_{j,\C}<\epsilon$, which cannot occur. Lastly, if $p_{i,\C}>(1-\epsilon)\cdot\C$, then $p_{i,\C}>p^{*}_{i,\C}$. This implies that at least one of the other $N$ tokens is less than their fair value. 


\subsubsection{LP Strategy in an Individual Pool}
Suppose an LP wants to provide liquidity for the token pair $\K_{\textbf{j}}/\I$ for some $\textbf{j}\in [1,N]$. Suppose the current price of the above pair is $p$ satisfying:
\begin{equation}
 \frac{\epsilon}{N(1-\epsilon)}< p< \frac{1-\epsilon}{N\epsilon}.   
\end{equation}
Then, the LP can choose to deposit $\I$

==> instructions.tex <==
\section{Ease of Use}

\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.


==> notes.tex <==
\section{Notes}
Let's understand the difference between having N pairs of $K_{i}/I_{i}$ vs having a single $I$ for the N pairs:
\begin{enumerate}
    \item The first part is straightforward: you create a marketplace for each binary option using conc-liquidity. You need zero additional capital for liquidity provision since the pair is $K_{i}/I_{i}$ and does not require $C$. Yes, there will be too many pairs, but so what? It remains capital-efficient. The only down-point is that it is not too fancy for a paper.
    \item On the other hand, you use DEEPER, which looks fancy. But is it really required?
\end{enumerate}
\textbf{Decision:} It has been decided that we will have a simple binary option-based insurance, no deeper. We will have another paper as a journal extension that will include deeper.

\if 0
An important consideration for such a marketplace is capital-efficient liquidity provision \emph{i.e.,} providing higher liquidity using same amount of asset reserves. Therefore, we propose using a shared concentrated liquidity DEX such as \textbf{DEEPER (put it as an add-on otherwise, reviewers might not understand the paper)} on the $N$ trading pairs $\K_{i}/\I$ with $\I$ being the common token. Compared to having $N$ separate pools, one for each trading pair $\K_{i}/\I$, the shared liquidity model enhances the liquidity of $\I$.
\fi

Lastly, one can also consider consolidating \TODO{You killed me here, your claim most likely is another paper worth of material to substantiate it
but again I am lost by this point, but this is the impression you give me.} multiple related adversities within a single Oracle contract. For example, a single $\K/\I$ token pair could effectively model the de-pegging of a collection of stable assets. In this context, $\K$ compensates if any one of the assets de-pegs, thereby minimizing the capital required from the underwriters ($\I$ holders).

Can write incentivation and kleros in discussion as well.

Unable to distinguish the related work and the contributions by the author. Authors should explain more about the background of DeFi and the exact problem they are solving, but it seems authors have assumed that the readers have the knowledge of finance and dives directly into technical details. Also the paper is losely related to Blockchain conference, more of a maths or economics paper.
